An Experimentation Infrastructure for Quantitative Measurements of Cyber Resilience

The vulnerability of cyber-physical systems to cyber attack is well known, and the requirement to build cyber resilience into these systems has been firmly established. The key challenge this paper addresses is that maturing this discipline requires the development of techniques, tools, and processes for objectively, rigorously, and quantitatively measuring the attributes of cyber resilience. Researchers and program managers need to be able to determine if the implementation of a resilience solution actually increases the resilience of the system. In previous work, a table top exercise was conducted using a notional heavy vehicle on a fictitious military mission while under a cyber attack. While this exercise provided some useful data, more and higher fidelity data is required to refine the measurement methodology. This paper details the efforts made to construct a cost-effective experimentation infrastructure to provide such data. It also presents a case study using some of the data generated by the infrastructure.

==> auxiliary/PaxHeader/definitions.tex <==
30 mtime=1652157807.234205374
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2MjczYzc5YTtTYWZhcmk7RDkzODMwMjMtRjRDRi00NjdFLTgyRDAtNDAzOTBDMDA0OUU1
95 SCHILY.xattr.com.apple.quarantine=0083;6273c79a;Safari;D9383023-F4CF-467E-82D0-40390C0049E5


==> auxiliary/PaxHeader/graphics.tex <==
30 mtime=1652475761.531826988
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2MjczYzc5YTtTYWZhcmk7RDkzODMwMjMtRjRDRi00NjdFLTgyRDAtNDAzOTBDMDA0OUU1
95 SCHILY.xattr.com.apple.quarantine=0083;6273c79a;Safari;D9383023-F4CF-467E-82D0-40390C0049E5


==> auxiliary/PaxHeader/graphics_B0.tex <==
30 mtime=1652305120.226764451
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2MjczYzc5YTtTYWZhcmk7RDkzODMwMjMtRjRDRi00NjdFLTgyRDAtNDAzOTBDMDA0OUU1
95 SCHILY.xattr.com.apple.quarantine=0083;6273c79a;Safari;D9383023-F4CF-467E-82D0-40390C0049E5


==> auxiliary/PaxHeader/packages.tex <==
30 mtime=1652847359.269511837
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2MjczYzc5YTtTYWZhcmk7RDkzODMwMjMtRjRDRi00NjdFLTgyRDAtNDAzOTBDMDA0OUU1
95 SCHILY.xattr.com.apple.quarantine=0083;6273c79a;Safari;D9383023-F4CF-467E-82D0-40390C0049E5


==> auxiliary/PaxHeader/preamble.tex <==
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2MjczYzc5YTtTYWZhcmk7RDkzODMwMjMtRjRDRi00NjdFLTgyRDAtNDAzOTBDMDA0OUU1
95 SCHILY.xattr.com.apple.quarantine=0083;6273c79a;Safari;D9383023-F4CF-467E-82D0-40390C0049E5


==> auxiliary/PaxHeader/tables.tex <==
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2MjczYzc5YTtTYWZhcmk7RDkzODMwMjMtRjRDRi00NjdFLTgyRDAtNDAzOTBDMDA0OUU1
95 SCHILY.xattr.com.apple.quarantine=0083;6273c79a;Safari;D9383023-F4CF-467E-82D0-40390C0049E5


==> auxiliary/graphics_B0.tex <==
\newcommand\ff{\framebox}
\newcommand\fff{}
\newcommand\aaaaa[1]{\ff{\includegraphics[trim={55mm 27.5mm 50mm 35mm}, clip,width=15cm]{#1}}}
\newcommand\aaa[1]{\color{black}\fff{\includegraphics[width=0.98\columnwidth]{#1}}
\vspace{-1mm}}
\newcommand\ccc[1]{\fff{\includegraphics[trim={-10mm 0mm 0mm 0mm}, clip,width=1.2\columnwidth]{#1}}\vspace{-2mm}}
\newcommand\bbbbb[1]{\fff{\includegraphics[width=12.25cm]{#1}}}
\newcommand\bbb[1]{\fff{\includegraphics[width=0.95\columnwidth]{#1}}}
\newcommand\bb[1]{\fff{\includegraphics[width=0.2675\columnwidth]{#1}}}
\newcommand\bba[1]{\fff{\includegraphics[width=0.355\columnwidth]{#1}}}
\newcommand\bbzz[1]{\fff{\includegraphics[width=0.8025\columnwidth]{#1}}}
\newcommand\bbazz[1]{\fff{\includegraphics[width=0.99\columnwidth]{#1}}}
\newcommand\ggggg[1]{\fff{\includegraphics[width=10cm]{#1}}}
\newcommand\ccccc[1]{\ff{\includegraphics[trim={45mm 7.5mm 10mm 2.5mm},    clip,width=7cm]{#1}}}
\newcommand\eeeee[1]{\ff{\includegraphics[width=11cm]{#1}}}
% \newcommand\fffff[1]{\ff{\includegraphics[trim={55mm 27.5mm 50mm 3mm}, clip,width=15cm]{#1}}}
\newcommand\fffff[1]{\ff{\includegraphics[trim={55mm 27.5mm 50mm 3mm}, clip,width=10cm]{#1}}}
\newcommand\hhhhh[1]{ \fff{\includegraphics[height=3.125cm]{#1}}}
\newcommand\jjjjj[1]{ \fff{\includegraphics[width=6.5cm]{#1}}}
\newcommand\lllll[1]{\fff{\includegraphics[width=4.9cm]{#1}}}

\graphicspath{ {./figures/} }

==> includes/PaxHeader/abstract.tex <==
30 mtime=1652845706.988189691
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg0NTc5YztTYWZhcmk7QjNFREIyODAtNDUyQS00MTg4LTg3OUYtMDUyMzgxOTBCOTA4
95 SCHILY.xattr.com.apple.quarantine=0083;6284579c;Safari;B3EDB280-452A-4188-879F-05238190B908


==> includes/PaxHeader/analysis.tex <==
30 mtime=1652895990.808315688
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg1MmUzNTtTYWZhcmk7RTlERUNEQjQtMzQ0Mi00QTFCLTg0MzQtQTFBNjdFNEY3MzdF
95 SCHILY.xattr.com.apple.quarantine=0083;62852e35;Safari;E9DECDB4-3442-4A1B-8434-A1A67E4F737E


==> includes/PaxHeader/approach.tex <==
30 mtime=1652897102.929147416
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg0NTc5YztTYWZhcmk7QjNFREIyODAtNDUyQS00MTg4LTg3OUYtMDUyMzgxOTBCOTA4
95 SCHILY.xattr.com.apple.quarantine=0083;6284579c;Safari;B3EDB280-452A-4188-879F-05238190B908


==> includes/PaxHeader/background.tex <==
30 mtime=1652902825.695932881
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg1NGIxMDtTYWZhcmk7NTRBRjc2RjktN0ZBNi00OTJELUI4NEItNDNENUM4NzU5Q0RE
95 SCHILY.xattr.com.apple.quarantine=0083;62854b10;Safari;54AF76F9-7FA6-492D-B84B-43D5C8759CDD


==> includes/PaxHeader/introduction_a.tex <==
30 mtime=1652847873.587436001
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg0NTc5YztTYWZhcmk7QjNFREIyODAtNDUyQS00MTg4LTg3OUYtMDUyMzgxOTBCOTA4
95 SCHILY.xattr.com.apple.quarantine=0083;6284579c;Safari;B3EDB280-452A-4188-879F-05238190B908


==> includes/PaxHeader/introduction_b.tex <==
30 mtime=1652902815.844922129
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg1NGIxMDtTYWZhcmk7NTRBRjc2RjktN0ZBNi00OTJELUI4NEItNDNENUM4NzU5Q0RE
95 SCHILY.xattr.com.apple.quarantine=0083;62854b10;Safari;54AF76F9-7FA6-492D-B84B-43D5C8759CDD


==> includes/PaxHeader/symbols.tex <==
119 LIBARCHIVE.xattr.com.apple.quarantine=MDA4Mzs2Mjg0NTc5YztTYWZhcmk7QjNFREIyODAtNDUyQS00MTg4LTg3OUYtMDUyMzgxOTBCOTA4
95 SCHILY.xattr.com.apple.quarantine=0083;6284579c;Safari;B3EDB280-452A-4188-879F-05238190B908


==> includes/analysis_B0.tex <==
\section{Case Study Analysis}
Fig. 2 shows the observed fuel efficiency plotted over the mission duration. The light blue line represents the observed fuel efficiency under the baseline scenario during which no attacks took place. The dotted red line represents the fuel efficiency under the attack scenario, with an attack occurring at 450 s. The effects of the attack can be seen starting around 525 s, when the blue and red lines diverge. The loss of fuel efficiency, shaded orange, is the net effect of the attack on fuel efficiency. One way to describe the difference in performance between these scenarios is to compute the area under the fuel efficiency curves (AUC). Complicating that procedure is the observation that fuel efficiency in the attack scenario sometimes exceeds that under the baseline scenario after the attack has concluded. This behavior is a result of the fact that the engine coolant temperature takes an extended amount of time to get back up to normal operating temperatures from the $60^\circ\text{C}$ steady state observed while the fan controller is attacked. During this time period in the attack scenario, the fan is not needed. In contrast, the baseline scenario still regularly turns the fan on, during which its average fuel efficiency is adversely affected. Thus, a temporary period of increased average fuel efficiency is observed in the attack scenario. With this explanation, we may compute the AUC for the attack scenario as the minimum of the baseline and attack scenarios at each time point. The resulting loss in AUC due to the attack is 2\%.
In a second step, the experimental data were analyzed using the novel mathematical framework detailed in a companion paper [cite]. Briefly, the framework is used to express the functionality of a vehicle over mission time in terms of a parameterized change process. The key parameters are the impact  of malware and the impact  of so-called bonware (the totality of physical and cyber features that allow a system to resist and recover from cyber compromise). Since the effect of malware is not immediate, the effective onset of malware is modeled as an additional free parameter .
The process model is governed by the differential equation
\begin{equation}
  \frac{dF}{dt} = \left(\Fnominal-F(t)) \right) \bonware(t) - F(t) \malware(t) A(t) u(t-t^m),
\end{equation}
where $u(\cdot)$ is the unit step function, which takes the value 0 if its argument is negative and 1 otherwise.  indicates normative functionality and is set to 1 in this example.  is 1 if malware is active at time t and 0 otherwise.
The process is applied to the functionality  of the vehicle over mission time. Functionality at time  is defined as the ratio of a vehicular performance metric at time  in the experiment scenario divided by the same metric at time  in a baseline scenario that is free of malware. For the current example, we used fuel efficiency as the performance metric. Note that due to the high variability of fuel efficiency over short time intervals, the time series was first smoothed with a 72 s moving average window before taking the ratio.
The parameters of the model can be estimated from data using standard model fitting tools. Our implementation relied on the Monte Carlo estimation of a hidden Markov model as described in [cite]. For the current data, we estimated , , and  s. These model-based results allow us to quantify the relative impact of malware and bonware among different mission scenarios, vehicles, or attack and defense modalities.
Fig. 3 shows the functionality over time (solid light blue line) for the case study data. Also shown is the functionality predicted by the three-parameter differential equation model (dashed black line). The model captures the salient aspects of the data well
\begin{figure}
  \aaa{fuel_efficiency_1.pdf}
  \aaa{fuel_efficiency_2.pdf}
  \caption{Describe these fuel efficiency figures.}
\end{figure}


==> includes/analysis_OBSOLETE.tex <==
\subsection{Analysis}
The experimental data were analyzed using the novel mathematical framework detailed in a companion paper [cite].  Briefly, the framework is used to express the functionality of a vehicle over mission time in terms of a parameterized change process.  The key parameters are the impact $\malware$ of malware and the impact $\bonware$ of so-called bonware (the totality of physical and cyber features that allow a system to resist and recover from cyber compromise).  Since the effect of malware is not immediate, the effective onset of malware is modeled as an additional free parameter $t^m.$

The process model is governed by the differential equation \cite{Kott_mmcr} \begin{equation}\frac{dF}{dt} = (F_N-F(t)) B(t)-F(t) M(t) I(t) u(t-t^m),\end{equation}
where $I(t)=u(t^\text{i}-t)$ is an interaction term and $u(.)$ is the unit step function,
% $u(\tau)=\left\{ \begin{array}{cl} 0, & \tau <0\\1, & \tau\ge 0 \end{array} \right.$
which takes the value 0 if its argument is negative and 1 otherwise.  $F_N$ indicates normative functionality and is set to 1 in this example.

The process is applied to the functionality $F(t)$ of the vehicle over mission time.  Functionality at time $t$ is defined as the ratio of a vehicular performance metric at time $t$ in the experiment scenario divided by the same metric at time $t$ in a baseline scenario that is free of malware.  For the current example, we used fuel efficiency as the performance metric.  Note that due to the high variability of fuel efficiency over short time intervals, the time series was first smoothed with a 72 s moving average window before taking the ratio.

The parameters of the model can be estimated from data using standard model fitting tools.  Our implementation relied on the Monte Carlo estimation of a hidden Markov model as described in \cite{Kott_mmcr}.  For the current data, we estimated $\malware = 0.0102, \bonware = 0.0582,$ and $t^m = 525$ s.  These model based results allow us to quantify the relative impact of malware and bonware among different mission scenarios, vehicles, or attack and defense modalities.

\begin{figure}[h]
  \centering
  \aaa{fuel_eff.pdf}
  \caption{Caption}
  \label{fig:fuel:eff}
\end{figure}

Figure \ref{fig:fuel:eff} shows the functionality over time (solid light blue line) for the case study data.  Also shown is the functionality predicted by the three-parameter differential equation model (dashed black line).  The model captures the salient aspects of the data well.


\begin{figure}[h]
  \centering
  \aaa{fig_1.1.pdf}
  \aaa{fig_1.2.pdf}
  \caption{Route 1 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \aaa{fig_2.1.pdf}
  \aaa{fig_2.2.pdf}
  \caption{Route 2 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \aaa{fig_3.1.pdf}
  \aaa{fig_3.2.pdf}
  \caption{Route 3 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \aaa{fig_4.1.pdf}
  \aaa{fig_4.2.pdf}
  \caption{Route 4 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \aaa{fig_5.1.pdf}
  \aaa{fig_5.2.pdf}
  \caption{Route 5 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}



==> includes/approach.tex <==
\section{Approach}\label{sec:approach}

\subsection{Component Descriptions}
Multiple technologies have been integrated together to facilitate the
generation of realistic vehicle data.
In our experimentation setup, these include the \ac{PASTA} by Toyota,
the Unity game development platform, the \ac{ADF} developed in-house here
at the U.S. Army Research Laboratory,
and the OpenTAP test automation framework by Keysight Technologies.
In general, Unity generates messages via the \ac{MQTT} 
publish-subscribe network protocol.
\ac{ADF} ingests these messages and translates them to \ac{CAN} format,
which are then injected onto the appropriate \ac{CAN} bus within \ac{PASTA}.
Data flowing in the opposite direction is handled in a similar manner,
but in reverse. Fig.~\ref{fg:datamodel} illustrates the flow of data between
components.

\begin{figure}[htbp]
	\centerline{\includegraphics{figures/dataflow.png}}
	\caption{
		A high-level overview of the data flow between compnents.
		Protions are derived from \cite{toyama2018pasta}
	}
	\label{fg:datamodel}
\end{figure}

\subsubsection{Portable Automotive Security Testbed with Adaptability}
\ac{PASTA}, created by Toyota, is a vehicle security testbed designed to
allow researchers the ability to develop and evaluate new security technology
and approaches on realistic ``white-box'' \acp{ECU}\cite{toyama2018pasta}.
There are three vehicle \acp{ECU} within the testbed, each encompassing a
family of functionality and sitting on their own \ac{CAN} bus: powertrain,
body, and chassis.
These three \acp{ECU} are responsible for their respective group of messages,
each generating and responding to traffic on their bus.
A fourth \ac{ECU}, the \ac{CGW}, acts as a junction between the three
previously mentioned buses.
Based on the message and source bus, the \ac{CGW} ferries messages to their
appropriate destination bus.
The firmware for all \acp{ECU} is open-source, and is accompanied by an
\ac{IDE} from Toyota to promote ease of customization.

\ac{PASTA} has simulation boards integrated into the testbed which calculate
how the current \ac{CAN} messages on the buses would influence a commercial
sedan.
These boards then update the vehicle \acp{ECU} with appropriate values.
For example, when acceleration pedal operation is inputted, the chassis
\ac{ECU} sends a message with the indicated value as a percent.
The simulation boards observe this message and calculate the physics that
would result from the input.
The results are used to update the values reported by the powertrain \ac{ECU},
which it outputs onto its bus.
In this instance, the powertrain ECU would send messages indicating the new
engine throttle position, \ac{RPM}, and vehicle speed.
The simulation boards are connected directly to the vehicle \acp{ECU} via a
serial port on each ECU board, so the physics data is not mixed with messages
on the \ac{CAN} bus.

An issue with the simulation boards is that they are essentially
``black-boxes'' and closed-source.
We cannot alter, for instance, the parameters involving the engine (e.g.,
torque and horsepower), the weight of the vehicle, or the terrain that the
boards are assuming is being traversed.
To counteract this issue, we integrated a simulation engine that would allow
for user-defined vehicle details as well as a custom terrain.
In this configuration, \ac{PASTA} becomes hardware-in-the-loop for the
simulation engine.
Attacks or defenses that affect the \acp{ECU} present in \ac{PASTA} will also
affect the vehicle within simulation.
This is essential in order to observe realistic threats and defenses and
their effects on vehicle performance.

\subsubsection{Unity}
Unity is a widely-used multi-platform game development platform implemented
in C\#\cite{unity2021unity}.
It includes out-of-the-box tools, assets, and an \ac{IDE} to aid developers
in creating 3D designs and models.
In particular, Unity provides built-in assets and classes regarding vehicle
physics, which we leverage to model interactions between our simulated
vehicle and custom terrain.

\paragraph{Simulated Light Military Vehicle}
We implemented a light military vehicle within Unity designed to interface
with data inputs from the white-box \acp{ECU} within \ac{PASTA}.
In general, the vehicle produces inputs in response to the simulated terrain.
These inputs are sent to the corresponding \acp{ECU} within \ac{PASTA} as if
they were generated by \ac{PASTA} itself.
We then send responses to these inputs from the \acp{ECU} back to the
simulated vehicle, which it uses to calculate things like torque and fuel
consumption.
For example, assume that the vehicle reports that the accelerator is set to
50\%.
This message is injected into \ac{PASTA} as if the chassis \ac{ECU} had
generated it.
The powertrain ECU responds to the message with the corresponding amount of
engine throttle.
A message with the engine throttle is sent back to the vehicle, which is then
applied to engine power calculations.
With this data flow, any attacks present on the \ac{ECU} within \ac{PASTA}
will affect the simulated vehicle.

An automated driver is responsible for generating steering, acceleration,
and braking inputs as the vehicle traverses the simulated terrain.
Steering is guided by the use of a waypoint system.
Both acceleration and braking inputs are calculated via a
\ac{PID} controller.
The controller reliably responds to sudden changes in the terrain or vehicle
performance, and maintains the target vehicle speed while preventing
oscillation around the target vehicle speed.

Engine performance is calculated through the use of torque, horsepower, and
\ac{BSFC} curves.
Engine RPM is derived using the vehicle speed, wheel circumference, and
effective gear ratio.
Using this \ac{RPM} value, the curves are evaluated to discern the
corresponding torque, horsepower, and \ac{BSFC} value.
Torque is multiplied by the throttle and the current effective gear ratio to
obtain the total amount of torque that can be applied to the wheels.
Since our vehicle is  \ac{AWD}, each wheel receives the total amount of
torque divided by the number of wheels on the vehicle, which is six in this
case.
Horsepower and the \ac{BSFC} value are used in conjunction to calculate the
amount of fuel that has been used.
Based upon the torque curve as a whole, gear shift points were calculated
manually.
The resulting shift points, being optimal in terms of torque output, confer
an aggressive acceleration profile for the vehicle.
Appendix A
contains formulas used to calculate the engine \ac{RPM}, the total current
torque, and fuel consumption at each update of the physics engine.

The vehicle is capable of providing sensor information that is either not
present in \ac{PASTA} or needs its functionality altered for our purposes.
Currently, this applies to the engine coolant temperature.
Engine temperature is present in \ac{PASTA}, but is aligned to the
temperature characteristics of a commercial sedan.
Within Unity, we implemented a basic temperature model that can be controlled
by an external fan controller \ac{ECU}.
The fan controller, described in a later section, monitors the coolant
temperature reported by the vehicle.
Once it reaches an upper threshold limit, it activates the simulated fan on
the vehicle, which begins to lower the temperature to an acceptable lower
threshold.
The fan itself takes around 50 horsepower to operate, which results in an
approximate 25\% drop in the available torque that can be applied to the
wheels.

\paragraph{Terrain}
The simulated vehicle within Unity traverses a custom terrain map that is
roughly 81.8 km by 100 km with altitudes up to 910 m.
We crafted a course approximately 151 km in length across the map that
encompasses multiple terrain types: flat main road, float off-road, hilly,
prolonged incline, and prolonged decline.
We placed trigger points on the map that set the target speed of the vehicle
depending on the terrain type.
If on a flat main road, the target speed is 60 km per hour.
Otherwise, the target speed is 40 km per hour

\paragraph{Reportable Data}
***Working on it***

\paragraph{Active Defense Framework}
\ac{ADF} is a government-developed framework used to rapidly prototype
network-based active cyber-defense techniques.
\ac{ADF} currently supports \ac{IP} networks and vehicle control networks,
namely the \ac{CAN} bus and Society of Automotive Engineers J1708 bus,
respectively.
The framework itself is written in Python and C programming languages,
while active cyber-defense plugins can be written in Python.
The framework acts as an intermediary for network traffic, as depicted in
Fig.~|ref{fg:dataflow}, allowing it to control network message flow, as well
as inspect, modify, drop, or generate network messages.
Essentially, the plugin developer has free reign to prototype any
network-based cyber-defense or detection technique they can imagine. 

\ac{ADF} is a fully modular architecture comprising the core framework and
plugins.
The main framework process is responsible for managing plugins and handling
events, but it does not play any role in packet processing, and it can handle
any type of packet- or message-based traffic. 

Each plugin is a self-contained module.
Plugins are linked by the framework based on the configuration.
Packets arrive at a plugin with information (a dictionary of attributes)
generated by the previous plugins.
After taking some action on the packet or the information, the packet is
dispatched to other plugin(s) based on the configured links and the packet
information.
Specialized plugins are used to send and receive traffic via network
interfaces, buses, and other ADF instances.
By creating the proper plugins and linking them, ADF can act as a firewall,
bridge, gateway, or honeypot.

Each plugin can maintain state data.
The state of all plugins can be automatically saved and loaded by the
framework to provide persistence. 

Plugins communicate with each other by generating events, which are placed
into the framework’s event queue.
The framework pulls events from this queue and notifies the plugins in a
configurable order.
Each plugin can contain logic to modify the event or act based on it.

\ac{ADF} is used here to provide a system/software-in-the-loop capability,
and to provide simulated components.
It allows communication between \ac{PASTA} and Unity by translating \ac{CAN}
messages to and from \ac{MQTT}, a standard \ac{IP}-based messaging protocol.
\ac{ADF} plugins are also used to provide simulated \ac{ECU} hardware, and to
implement attack and defense methods on the CAN bus via ADF’s ability to
monitor, modify, inject, or drop CAN traffic.

\paragraph{Unity-to-PASTA Message Translation}
\ac{ADF} runs on a standalone laptop and is connected to \ac{PASTA} via two
\ac{USB} \ac{SLCAN} interface modules.
One module (can0) is connected to the powertrain \ac{CAN} bus, and the other
module (can1) is connected to the chassis CAN bus.
The \ac{PASTA} \ac{CGW} is disconnected from the CAN buses for this
experiment, and the body \ac{CAN} bus (along with the body \ac{ECU}) is not
used.
\ac{ADF} is configured to serve as a \ac{CGW} between Unity and \ac{PASTA},
but unlike the \ac{PASTA} \ac{CGW}, \ac{ADF} does not relay messages between
the powertrain and chassis \ac{CAN} buses.
\ac{ADF} relays powertrain \ac{CAN} messages to and from Unity and sends
vehicle parameters from Unity to the chassis \ac{CAN} bus for display on the
\ac{PASTA} instrument cluster.

Unity has no ability to natively communicate with \ac{CAN} interfaces, so
\ac{ADF} translates \ac{CAN} messages in real-time to \ac{MQTT} messages.

\ac{PASTA} Engine \ac{CAN} messages are received from the physical can0
interface by the CANInterface plugin and decoded by a DBCDecoder plugin
configured to parse \ac{PASTA} \ac{CAN} messages.
The messages, now with populated signal info attributes, are fed to the
MQTTClient plugin.
The MQTTClient plugin is configured to publish the \ac{PASTA} Engine
\ac{ECU} brake and throttle position messages to the ``SimToVis'' \ac{MQTT}
topic, which Unity subscribes to.
Each \ac{MQTT} message is formatted as (timestamp,parameter\_name,float\_value),
for example: ``1.234,spn91,0.5'' would tell Unity \ac{SPN}91
(\ac{SAE} J1939 throttle position) is at 50\%.
 
Simultaneously, Unity publishes the vehicle state to the “VisToSim” \ac{MQTT}
Topic and the MQTTClient plugin subscribes to that topic.
The \ac{MQTT} message format is the same (timestamp,parameter,value) tuple,
and parameters indicating the simulated accelerator, brake, and steering
wheel positions are configured to generate the same signals the \ac{PASTA}
Chassis \ac{ECU} would normally generate.
These signals are encoded to \ac{CAN} messages by the DBCEncoder plugin and
sent to the CANInterface for transmission on the physical can0 interface to
the \ac{PASTA} Engine \ac{CAN}. 

The two-way \ac{CAN}-\ac{MQTT}-Unity channel serves the following purpose:
The control inputs to the Unity simulation (manual or automatic) simulate the
\ac{PASTA} Chassis \ac{ECU} providing inputs to the \ac{PASTA} Engine
\ac{ECU}, and the Unity vehicle responds based on the throttle position and
brake system operation outputs from the \ac{PASTA} Engine \ac{ECU}. 

A second MQTTClient subscribes to the VisToSim topic and translates the
simulated vehicle speed, \ac{RPM}, and coolant temperature values to \ac{CAN}
messages that would normally be generated by the \ac{PASTA} Engine \ac{ECU}.
These messages are sent on the Chassis \ac{CAN} bus for display on the
\ac{PASTA} instrument cluster.
This ensures the \ac{PASTA} instruments reflect the simulated vehicle in
Unity, and that any real or simulated \acp{ECU} we add to the \ac{PASTA}
Chassis \ac{CAN} bus receive the simulate vehicle signals.

\paragraph{Virtual \acp{ECU} within \ac{ADF}}
The \ac{PASTA} platform does not simulate a controllable cooling fan or
provide a fan controller \ac{ECU}.
Therefore, we simulate a fan controller \ac{ECU} using \ac{ADF}.
The fan controller needs to engage the engine cooling fan when the engine
coolant temperature reached a defined threshold and disengage the cooling fan
when the coolant temperature drops below a defined threshold.
Additionally, for the purposes of this experiment, we need to simulate an
attack on this \ac{ECU}’s firmware that would force the fan to remain on
indefinitely, and reset the \ac{ECU} to restore normal operation.

An \ac{ADF} plugin was developed to simulate this engine fan controller
\ac{ECU}.
The \ac{ECU} is attached to the \ac{PASTA} Chassis \ac{CAN} bus and listens
for \ac{PASTA} engine temperature \ac{CAN} messages
(P\_ENGINE\_TEMP, \ac{CAN} ID 387).
It generates a fan control message (C\_FAN, \ac{CAN} ID 388) once per second.
The fan control message is ignored by \ac{PASTA} but is published by the
MQTTClient as the ‘fan\_control’ parameter via the ``SimToVis'' \ac{MQTT}
topic.

In normal operation, the fan controller sends C\_FAN message with
fan\_control=0 until the coolant temperature is reported as 103 degrees
Celsius or higher.
At this point, C\_FAN messages are sent with fan\_control=1 until the
reported temperature drops to 85 degrees Celsius or lower.
The Unity simulation responds to the fan\_control parameter by gradually
raising the temperature if it is 0, or lowering it if it is 1.
As long as the fan control ECU is receiving the correct coolant temperature
signal and operating normally, the coolant temperature will remain in the
vehicle's operating range after it has initially warmed up. 

For attack and defend experiments, the fan controller \ac{ADF} plugin can
respond to trigger events to simulate an attack, stop the simulated attack,
or reset itself.
During a simulated reset, the fan controller is offline and does not produce
C\_FAN messages for 20 seconds.
A watchdog routine is included in the simulated \ac{ECU} to detect abnormal
behavior: If, after vehicle warm-up, the coolant temperature remains outside
of the normal operational range for more than 100 seconds plus or minus a
random window, an \ac{ECU} reset will be automatically triggered.

\paragraph{Attack Possibilities via \ac{ADF}}
The simplest attack on a vehicle bus is to inject messages.
Messages are broadcast on a \ac{CAN} bus, so a message injected at any point
on the bus will reach all \acp{ECU} on the bus.
While an injection attack cannot block or modify the normal \ac{CAN} bus
traffic, it can impact vehicle performance if we can we inject messages that
cause constant undesired vehicle behavior.
For example, in heavy vehicles a \ac{PGN} 0 message is emitted by an \ac{ECU}
that needs to control the engine speed or output torque.
Normal sources of \ac{PGN} 0 include the brake controllers when loss of
traction is detected, and the automatic transmission controller when the
engine torque/speed needs to be reduced to safely shift gear.
If a \ac{PGN} 0 message demanding idle speed or torque is continually
injected on the bus, the engine will be forced to idle and the accelerator
will be unresponsive.

If an attacker can physically sever the \ac{CAN} bus wiring at a strategic
point and place additional hardware at that point, it is possible to modify
the normal bus traffic.
Attacks that block or modify messages can prevent \ac{ECU} from controlling
the vehicle or falsify vehicle data. One example would be reporting a lower
than actual coolant temperature, preventing the fan from engaging and
eventually causing the engine to overheat.
Another example would be blocking legitimate \ac{PGN} 0 control messages,
which would disable traction/stability control or prevent the transmission
from shifting.	

Attacks on \ac{ECU} firmware, by embedding malware, are also feasible.
Malware on the fan controller is simulated by sending a trigger event to the
\ac{ADF} plugin.
The attack we simulated is a ``stuck fan'' attack in which malware has
modified the fan control \ac{ECU} to not disengage the fan once engaged,
even when the coolant temperature has dropped below the minimum operational
temperature.
This does not result in an immediately noticeable condition such as
overheating, but will reduce powertrain output and increase fuel consumption.

\paragraph{Defensive Capabilities via \ac{ADF}}
Defending against message injection at the bus level requires detecting and
filtering injected messages before they reach the \ac{ECU}.
The \ac{CAN} bus can be split at potential access points and hardware placed
in-line, as with the blocking/modification attack.
Alternatively, hardware can be placed between the \ac{CAN} bus and critical
\acp{ECU}, or defenses can be integrated into the \ac{ECU}.
These types of defenses can also detect and block modified messages.

Detection of injected or modified messages can be achieved by watermarking
valid messages.
A cryptographic watermark can be inserted into the reserved or
least-significant bits of a message before it traverses the bus and verified
by recipients.
Alternatively, messages can be cryptographically signed, and the signature
transmitted as an additional message.
Messages injected or modified by the attacker will not have a valid watermark
or signature and will be rejected. 

Message blocking or modification can also be detected by modeling the vehicle
based on observable state and comparing the parameters in the suspect message
to the model’s prediction.
Additionally, if messages are being blocked, or messages with invalid
watermarks/signatures are rejected, those messages need to be generated.
For example, coolant temperature can be modeled based on intake air
temperature, fuel temperature, and oil temperature.
If the coolant temperature message is missing or not within range of the
prediction, we can substitute a message containing the predicted coolant
temperature. 

These defenses deal with bus-level attacks, not attacks on the \acp{ECU}.
If an \ac{ECU} is compromised, measures must be taken to restore proper
\ac{ECU} function.
Many \acp{ECU} can be reset or ``re-flashed'' (\ac{ECU} firmware replaced)
while the vehicle is operational.
The \ac{ECU} may or may not be functional for some duration while being reset
or re-flashed, and the impact this will have to vehicle performance depends
on the function of the \ac{ECU}.
For the \acp{ECU} simulated by ADF plugins, the behavior is to make the 
\ac{ECU} unresponsive for a set duration, after which normal \ac{ECU}
operation is restored.

\subsubsection{OpenTAP}
***Working on it***

%%%     \subsection{Illstrative Case Study}
%%%     We created and ran an experiment scenario wherein malware has infected the
%%%     fan controller \ac{ECU} present on the vehicle.
%%%     Possible infection vectors could include either a tainted supply chain or an
%%%     infected technician computer used during regular maintenance of the vehicle.
%%%     Once active, the malware removes the ability to disengage the engine coolant
%%%     fan from the fan controller \ac{ECU}.
%%%     This causes the vehicle to enter a state of prolonged degraded performance
%%%     due to the fact that the engine coolant fan draws approximately 25\% of the
%%%     available horsepower in order to operate.
%%%     Note that we did not employ actual malware in this experiment.
%%%     We simulated the effects of the malware and applied them to the fan controller
%%%     \ac{ECU} implemented within ADF. 
%%%     
%%%     The experiment runs for 800 seconds, with the attack commencing around 450
%%%     seconds from the start of the run.
%%%     Bonware present on the vehicle monitors the engine coolant temperature for
%%%     any abnormalities.
%%%     From this sensor reading, it will notice the effect of the malware and
%%%     attempt to recover after a period observation to ensure the behavior is not
%%%     a short-lived anomaly.
%%%     Recovery from this attack consists of re-flashing the firmware on the fan
%%%     controller \ac{ECU}.
%%%     On an actual \ac{ECU}, this process takes approximately 20 seconds to
%%%     complete.
%%%     Since our fan controller is implemented within \ac{ADF}, this process is also
%%%     simulated.

==> includes/background.tex <==
\section{Background}\label{sec:background}
This section will be provide a summary of some of the key issues.
A scientific definition of cyber resilience is necessary for a quantitative
measurement.
Although this topic deserves serious consideration, which will be provided in
a subsequent work, a brief overview is provided.
A brief explanation of the method used to measure cyber resilience is 
provided, and a more detailed review of the literature may be found
in \cite{smith2022quantitative}.
The literature is reviewed for previous work on vehicle simulators for
cyber research.

\subsection{Definition of Cyber Resilience}
As Locke observes, ``A valid definition of a concept is a prerequisite to
valid measurement.''\cite{locke2003good}
However, there are many definitions of resilience and cyber resilience in
the literature.
``One expert claims that well over 100 unique definitions of
resilience have appeared.''\cite{brtis2019systems}
Several systematic reviews of the literature looking for a consensus on the
definition for resilience came the same conclusion.
There is no consensus on the definition of resilience.\cite{
	klein2003resilience,
	wald2006literature,
	norris2008community,
	reid2013multiple,
	woods2015four,
	aburn2016resilience,
	arghandeh2016definition,
	xue2018exploring,
	cottam2019defining,
	beling2021developmental}
Many have gone so far as to say that the concept of resilience is on the 
precipice of becoming a meaningless buzzword.\cite{
	klein2003resilience,
    rose2007economic,
    reid2013multiple,
	hussain2013resilience,
	phillips2022rethinking,
	soubry2022you}
	
In an effort reign in the ever expanding definition of resilience and
perhapse salvage it from the ignominious fate of becoming a meaningless
buzzword, this paper will use a definition of resilience which goes back
to the root word resile.  The word resile means to jump
back.\cite{oxford1993resile}  Before Holling began its
expansion,\cite{holling1973resilience} the concept of resilience was
defined as the amount of stress that could be absorbed
elastically.\cite{
	oxford1993resilience,
	bodin2004resilience,
	american2006resilience,
	norris2008community,
	reid2013multiple}
It described the ability of a spring to expand or contract
but still return to the original shape.
It is measured in Pascals.

A definition of cyber resilience based upon the definition of resilience
in material science would provide something like, ``cyber resilience is
defined as the ability of a cyber system to recover its performance after
an unwanted degradation.''
Key to this concept is that resilience under this definition is not only
about systems where the performance does not degrade.
That is resistence.
Certanly that is a laudable goal; however, it has already been acknowleged
that perfect security is impracticle.
Secondly resilience under this definition is not only about systems that
degrade, but provide enough functionality to complete the mission.
That is toughness.
This goal may be accomplished by over engineering the article.
Under this definition resilience is about recovery.
It requires either cessation stress either because the system has left
the area of influence of the stressor or because the system has healed
itself and removed the stressor.
This second method is the subject of Kott and Theron's call for intelligent
autonomous agents.\cite{kott2020doers}
These intelligent autonomous agents will be called ``bonware'' as the 
operate in opposition to ``malware''.

\subsection{Measurement of Cyber Resilience}
If we had a method for quantitatively measuring cyber stress, a quantitative
measurement for cyber resilience would be straight forward.
Until further research can define what a cyber Pascal is and how to measure
it, we will need some other method.
In this experiment we will measure cyber stress by measuring the degradation
of a system's \acp{KPP} under stress.
In this experiment will measure
This would be similiar to measuring the amount of stretch in a spring to
deterime weight.

Ligo et al.\cite{ligo2021measure} surveyed various measurement
techniques for cyber resilience in their paper,
``How to Measure Cyber Resilience of an Autonomous Agent:
Approaches and Challenges.''\cite{ligo2021measure}
They propose plotting the performance of a system under cyber-attack
and measuring the area under the curve, as seen in
Fig.~\ref{fig:curve}.

\begin{figure}[h!]
	\includegraphics[width=3.5in]{figures/curve.png}
	\caption{
		Representation of resilience as the area under the curve
		of systems functionality over time as presented by Ligo
		et al.\cite{ligo2021measure}
	}
	\label{fig:curve}
\end{figure}

In his report, ``How to Think About Resilience in a \ac{DoD}
Context\cite{brtis2016think},''
Brtis recommends a framework for addressing resilience in military systems.
This framework includes a metric for measuring resilience.
``We evaluated 23 candidate metrics against 19 evaluation criteria.
From this analysis we conclude that the best single metric for
resiliency is the expected availability of the required
capability.''\cite{brtis2016think}

\subsection{Experimental Environments}
Much of the early work on the cybersecurity of automobiles was done using
actual vehicle.\cite{hoppe2007sniffing,foster2015fast}
This provides the most fidelity; however, it is very expensive to conduct
research in this fashion.
The number of run required to generate the data necessary to validate a 
quantitative measurement of cyber resilience would be prohibitively
expensive. 

Some researchers conducted research by connecting multiple \acp{ECU} together
on a \ac{CAN} bus independent of a
vehicle.\cite{daily2016towards,bozdal2018hardware}
These do indeed provided an inexpensive method to test malware and bonware
in a vehicular network; however, they cannot capture impacts on the 
vehicle's \acp{KPP}.

\cite{wang2018delay}

\cite{stachowski2019cybersecurity}

Digital twin\cite{shikata2019digital}




==> includes/component_description.tex <==
\section{Component Description}
Multiple technologies have been integrated together to facilitate the
generation of realistic vehicle data. In our experimentation setup,
these include the Portable Automotive Security Testbed with
Adaptability (PASTA) by Toyota, the Unity3D game development engine,
the Active Defense Framework (ADF) developed in-house here at the Army
Research Laboratory, and the OpenTAP test automation framework by
Keysight Technologies. In general, Unity3D generates messages via the
MQTT publish-subscribe network protocol. ADF ingests these messages
and translates them to CAN format, which are then injected onto the
appropriate CAN bus within PASTA. Data flowing in the opposite
direction is handled in a similar manner, but in reverse. Figure \ref{fig:1}
illustrates the flow of data between components.

\begin{figure}[h]
  \centering
  \aaa{figure_1.pdf}
  \caption{A high-level overview of the data flow between components. Portions of Fig. 1 are derived from \cite{toyama}}
  \label{fig:1}
\end{figure}


==> includes/counter_cyber.tex <==
\section{Current counter cyber technology/efforts}
Modern vehicles (since the 1980s) use a network of electronic modules for command, control and data sharing among the various vehicle systems like the instrument cluster, engine and transmission. This network configuration is loosely analogous to general purpose networks where a number of computers are linked together typically for data sharing but also command and control. Because of this vehicle cyber security has grown from and is considered to be a branch of the wider cyber security industry. As such many of the tools are derived from those used in general purpose computer networks. Vehicle cyber security tools include:
\begin{itemize}
  \item Data Traffic Pattern Analysis (Detection) – In this technique the assumption is made that data traffic on the vehicle network absent external or malicious inputs will follow regular message patterns that can be used to detect cyber threats when the patterns are thrown off \cite{nrel}.
  \item Canary/Honey Pot (Detection) – In this technique a device is set up in the vehicle network with perceived or known interest and vulnerabilities such that an attacker will be drawn to it. The vulnerabilities in the device by design represent no actual threat to the larger system. The cyber security system can intensively monitor this sub system for activity \cite{canary}.
  \item    Fingerprinting (Detection) – In this technique the unique physical layer electrical signature of each component on the vehicle network is known to a monitoring system. Any attempt by an unauthorized device can be detected because of its electrical signature and any otherwise authorized device sending messages that it is not approved to send can also be detected.
  \item Traffic Rate Monitoring (Detection) – Looking at the rates at which certain vehicle network traffic components are broadcast and comparing this to expected values. This can be used to detect traffic overload attacks.
  \item    Traffic Contextualization (Detection) – In this technique the vehicle network traffic is validated against a set of rules that looks for contextually inappropriate traffic like stationary maintenance functions being launched during moving vehicle operations.  
  \item Access Firewalling (Detection \& Protection) – In this technique vehicle network access points are firewalled until a password or other is received by a connecting device.  
  \item Man In The Middle (MITM) (Detection \& Protection) – In this technique a cyber protective module is put in front of, or built into, every critical vehicle module. MITM can be used to host detective cyber security tools and provide a protective filtering of malicious messages. MITM can also be used to encrypt some or all data bus message traffic \cite{nhtsa}.
  \item Message Destructors (Detection \& Protection) – In this technique a single cyber protective module is put on the vehicle network. A message destructor can be used to host detective cyber security tools and actively delete malicious messages on the data bus by electrically altering certain parts of a message that will cause it to fail validation.
  \end{itemize}
  Vehicle networks tend to differ from general purpose computer networks in the use unauthenticated message traffic driven by the need for real time critical command and control messaging. Most general purpose networks will require authentication before allowing message traffic to flow into nodes. This authentication is a natural point to implement cyber security. In addition, while the applications that run on general purpose networks can be very comprehensive, the code base runs on a limited variety of operating systems that can be monitored for irregularities by a broad and sophisticated industrial base of cyber security expertise. Many vehicle networks use single message commands that come from highly proprietary embed applications with a wide variety of known and unknown vulnerabilities and with only ad hoc attention to cyber security. Because there is no enforced authentication, any compromised system on a vehicle network can be widely used to propagate threats with real time consequences.
When used together and implemented in a way that reflects the more application specific aspects of the vehicle cyber threat space, the tools listed can be effective. When used in a manner that is relevant for general purpose computer networks but not the vehicle networks these tools can end up only providing a token level of protection.
There are a number of companies providing vehicle cyber security solutions (NVIDIA, Harman, IBM, Dellfer, DENSO, etc.). Each company uses a selection of cyber security tools including some of the techniques listed. The problem is there is currently no method to evaluate how resilient each solution is to even the minimalist known threat space.
\subsection{Cyber threats: focus areas, types and nature}

The vehicle network threats for MGVs (Military Ground Vehicles) can be broken into three focus areas:
\begin{itemize}
  \item Mobility Threats
    \begin{itemize}
    \item a vehicle will not function because a cyber-originated threat renders the vehicle unable to start or incapable of moving.
    \item      a vehicle cannot be controlled by the operators because a cyber-originated threat takes control of certain vehicle functions like the accelerator pedal or transmission gear selection.
    \item      a vehicle suffers immobilizing or damaging incident because of a cyber-originated threat. Using an accelerator pedal control to cause a mishap would be an example of this.
    \end{itemize}
  \item Observability Threats\\
PLI (Position Location Information) identification is enabled because a cyber-originated threat turns on an energy emitting vehicle system that makes the vehicle more detectable to a red force. Inappropriately turning on headlights or window grid heaters would be an example of this.
\item Weapons Employment Threats\\
  a weapons system cannot be used because a cyber-originated threat renders the weapons system inoperable. A threat that inappropriately engages a weapons system safety interlock would be an example of this.
  \end{itemize}
The focus areas listed only cover how the threats impact the vehicle. They say nothing about the nature of the threats or how they are implemented in the vehicle network. If the same threat category (for example a single message command attack) can be used to cover all three areas any evaluation of resiliency will have limited utility because the available threat space is much wider than what is being evaluated. In order for the evaluation to be valid it must also span the type and nature of possible vehicle network threats including:
\begin{itemize}
  \item Vehicle Network Threat Types
    \begin{itemize}
      \item Industry wide vehicle network open standard messages (SAE, ISO, etc.) that can be misused to initiate vehicle network threats.
        \begin{itemize}
          \item Engine power output control  (SAE PGN0)
          \item Cooling control (temperature message rate over broadcast degrading cooling system performance)
          \item Chassis pitch yaw sensor accuracy (message rate over broadcast using inaccurate data effects weapons systems performance)
          \item Neutral safety violation (no engine start)
          \end{itemize}
          \item Manufacture proprietary vehicle network messages that can be used to initiate vehicle network threats.
            \begin{itemize}
            \item Lighting control (turn on lights identifying blue force location)
            \item Window heater control (turn on grid heater = increased vehicle IR signature)
            \item Transfer case control (range shift while moving causes catastrophic failure)
            \item Suspension control (ride height imbalances causes restricted performance limp home mode operation)
            \item Brake functionality (message interference cause brake performance issues)
            \end{itemize}
          \item Manufacturer diagnostic packages that use specific purpose vehicle network messages for testing. Many of these messages can be repurposed to initiate vehicle network attacks.
            \begin{itemize}
              \item Tire pressure control (unintended inflation/deflation)
              \item Data bus gateway control (message routing failures between data networks causing any number of issues)
              \end{itemize}
            \item Zero day (otherwise unknown) vehicle network threats that are discovered by network scanning, penetration testing, flash file decoding and analysis.
            \end{itemize}
          \item Vehicle Network Threat Natures
            \begin{itemize}
            \item Single message vehicle network attacks.
            \item Repeated message single vehicle network attacks.
            \item Sequenced of messages vehicle network attacks
              \item Module reprogramming on the vehicle network to embed triggerable threats
            \end{itemize}
          \end{itemize}

\subsection{Implementing cyber threats on desktop systems like Toyota PASTA}

Toyota PASTA (Portable Automotive Security Testbed with Adaptability) is a desktop system that emulates a functioning vehicle data network using various preprogrammed modules and a range of operator inputs to these modules. PASTA is meant to emulate vehicle networks found on civilian light vehicles, such as cars. The modules take the operator inputs and use these to generate vehicle network messages that reflect what would typically be seen on an operating vehicle. As such it has a library of defined messages many of which are similar to what is seen on MGVs. Because of this many of the cyber threats that can be implemented on MGVs can also be implemented on PASTA.  
This section will list a number of MGV on-vehicle threats along with a basic description of how each threat could be implemented on the PASTA table top system. Using the predefined messages in PASTA allows development and demonstrations of QMoCR that are not limited to actual physical MGVs. In cases where there is no realistic functional equivalency to an actual MGV, new control modules were adapted to work with PASTA to support enhanced testing.

\subsection{Mobility Threats}

\subsubsection{Threat - Throttle takeover (PGN 0)}
This attack gets its name from the message description for this function in SAE J1939-71. PGN 0 is intended to be used for normal engine control but can be abused by attackers. This type of attack takes control of the throttle from the operator. It can be maliciously used to send the engine power anywhere from full throttle to forced idle. It is performed by sending a repetitive throttle override message on the vehicle network.  This threat message is widely understood and normally used by traction control systems, torque limit requests during shifting by the transmission and other vehicle systems like pumps that require independent or override throttle control.\cite{truckhack}.  PASTA Equivalent for Throttle takeover (PGN 0) PASTA can use the message \texttt{SG\_ accelerator\_pedal\_operation\_indicator} to implement the same or similar functionality as PGN 0.  Threat - Deflate left front tire This type of attack takes control of the Central Tire Inflation System (CTIS) found on many MGVs from the operator. It can be maliciously used to send a deflate command message to any tire on the vehicle. For many CTIS equipped vehicles it is performed by sending a sequence of different messages on the vehicle network.  When actuated the tire will deflate and the operator can lose control of the vehicle or be forced to stop and attempt to rectify the condition.  This type of deflation event is normally used by CTIS laptop computer based diagnostics tool to troubleshoot problems with the system by independently actuating the system in ways that are not normally allowed.  PASTA Equivalent for Deflate left front tire Civilian vehicles (which PASTA represents) do not utilize CTIS. Adding a 3rd party module like CTIS to PASTA data bus would not alter the performance of a base system. So if a CTIS module was be added to PASTA system data bus, the same activation routine for the threat could be utilized.  Threat - Reprogram CTIS module firmware This type of attack reprograms the tire pressure targets of the Central Tire Inflation System (CTIS) found on many MGVs. It can be maliciously used to alter the tire pressure targets creating unsafe operating conditions (over-inflation/under-inflation) and poor vehicle performance in terrain. For many CTIS equipped vehicles it is performed by sending a sequence of proprietary messages on the vehicle network.  Since the CTIS system will purposefully track incorrect pressure targets when this threat is enabled the operator can lose control of the vehicle or be forced to stop and attempt to rectify the condition.  This type of event is normally used by CTIS laptop computer based diagnostic tool to reprogram the tire pressure targets based on solid engineering reasons and with the approval of the vehicle managers.  PASTA Equivalent for Reprogram CTIS module firmware Civilian vehicles (which PASTA represents) do not utilize CTIS. Adding a third party module like CTIS to PASTA data bus would not alter performance of the base system. So if a CTIS module was be added to PASTA system data bus and the same activation routine could be utilized.  Observability Threats

\subsubsection{Threat - Headlight activation}
This type of attack takes control of the headlights from the operator. It can be maliciously used to turn the headlights on or off. For many vehicles equipped with network connected headlight controls it is performed by sending a single command on the vehicle network. Since the operator loses control of visible light emissions when active it is considered an observability threat. Turning headlights on under certain conditions (night) can give a blue force vehicles location away to a red force.
This type of message is normally used by the headlight switch to operate the headlights over the vehicle network.
\subsubsection{PASTA Equivalent for Headlight Activation}
PASTA can use the message \texttt{SG\_headlight\_flashing\_switch} as relative near functional equivalent to the actual attack on an MGV. 
Threat - Front window defroster grid activation
This type of attack takes control of the front window heater grid (used for de-icing) from the operator. It can be maliciously used to turn the de-icer grid on or off. For many vehicles equipped with network connected window defroster grid controls it is performed by sending a single command set on the vehicle network. Since the operators loses control of thermal emissions when active it is considered an observability threat. Turning on a heat source under certain conditions can give away a vehicles location in infrared energy bands. Unlike turning on the normal lights the operators will not be aware this is occurring unless they have access to thermal viewing systems.
\subsubsection{PASTA Equivalent for Headlight Activation}
PASTA can use the message \texttt{SG\_horn\_switch} as the nearest functional equivalent to the actual attack on an MGV by simply relabeling the horn as the grid heater. 

\subsection{Weapons Employment Threats}

\subsubsection{Threat - Vehicle attitude sensor signal takeover}
This type of attack overrides the vehicle attitude sensor. It can be maliciously used to disable systems that require the vehicle to be level to a certain degree. For vehicles equipped with attitude sensors it is performed by sending a stream of messages on the vehicle network. Since the vehicle determines that it is oriented in a manner that exceeds weapons system limits they cannot be employed against targets.
This type of message flooding is never normally used but is not detectable by the current systems on the vehicle.
\subsubsection{PASTA Equivalent for Vehicle attitude sensor signal takeover}
PASTA can use the message for \texttt{SG\_ steering\_wheel\_operation\_position} as near functional equivalent to the actual attack on an MGV. 



==> includes/data.tex <==
\subsection{Analysis}

\begin{figure}[h]
  \centering
  \bbb{fig_1.1.pdf}
  \bbb{fig_1.2.pdf}
  \caption{Route 1 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \bbb{fig_2.1.pdf}
  \bbb{fig_2.2.pdf}
  \caption{Route 2 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \bbb{fig_3.1.pdf}
  \bbb{fig_3.2.pdf}
  \caption{Route 3 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \bbb{fig_4.1.pdf}
  \bbb{fig_4.2.pdf}
  \caption{Route 4 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

\begin{figure}[h]
  \centering
  \bbb{fig_5.1.pdf}
  \bbb{fig_5.2.pdf}
  \caption{Route 5 Baseline and Recovery}
  \label{fig:1.1}
\end{figure}

The experimental data were analyzed using the novel mathematical framework detailed in a companion paper [cite].  Briefly, the framework is used to express the functionality of a vehicle over mission time in terms of a parameterized change process.  The key parameters are the impact $\malware$ of malware and the impact $\bonware$ of so-called bonware (the totality of physical and cyber features that allow a system to resist and recover from cyber compromise).  Since the effect of malware is not immediate, the effective onset of malware is modeled as an additional free parameter $t^m.$

The process model is governed by the differential equation \cite{Kott_mmcr} \begin{equation}\frac{dF}{dt} = (F_N-F(t)) B(t)-F(t) M(t) I(t) u(t-t^m),\end{equation}
where $I(t)=u(t^\text{i}-t)$ is an interaction term and $u(.)$ is the unit step function,
% $u(\tau)=\left\{ \begin{array}{cl} 0, & \tau <0\\1, & \tau\ge 0 \end{array} \right.$
which takes the value 0 if its argument is negative and 1 otherwise.  $F_N$ indicates normative functionality and is set to 1 in this example.

The process is applied to the functionality $F(t)$ of the vehicle over mission time.  Functionality at time $t$ is defined as the ratio of a vehicular performance metric at time $t$ in the experiment scenario divided by the same metric at time $t$ in a baseline scenario that is free of malware.  For the current example, we used fuel efficiency as the performance metric.  Note that due to the high variability of fuel efficiency over short time intervals, the time series was first smoothed with a 72 s moving average window before taking the ratio.

The parameters of the model can be estimated from data using standard model fitting tools.  Our implementation relied on the Monte Carlo estimation of a hidden Markov model as described in \cite{Kott_mmcr}.  For the current data, we estimated $\malware = 0.0102, \bonware = 0.0582,$ and $t^m = 525$ s.  These model based results allow us to quantify the relative impact of malware and bonware among different mission scenarios, vehicles, or attack and defense modalities.

\begin{figure}[h]
  \centering
  % \bbb{fuel_eff.pdf}
  \bbb{fuel_efficiency_1.pdf}
  \caption{Caption}
  \label{fig:fuel:eff:1}
\end{figure}
\begin{figure}[h]
  \centering
  % \bbb{fuel_eff.pdf}
  \bbb{fuel_efficiency_2.pdf}
  \caption{Caption}
  \label{fig:fuel:eff:2}
\end{figure}

Figure \ref{fig:fuel:eff} shows the functionality over time (solid light blue line) for the case study data.  Also shown is the functionality predicted by the three-parameter differential equation model (dashed black line).  The model captures the salient aspects of the data well.



==> includes/introduction.tex <==
\section{Introduction}

Resilience is an important aspect of any cyber system.
A military system needs to be able to  resist, withstand and recover from an
attack without being compromised\cite{kott2019cyber}.
Security and management of risk are important, but they, in themselves,
do not guarantee resilience\cite{linkov2018risk}.
An unmanned military ground vehicle's controller area network (CAN) bus may
be compromised by malware, which effects the vehicles performance and may
actually result in an inability to complete its
mission\cite{bozdal2018august}. 

%%%     \subsection{Current counter cyber technology/efforts}
%%%     Modern vehicles (since the 1980s) use a network of electronic modules for %%%     command, control and data sharing among the various vehicle systems like the %%%     instrument cluster, engine and transmission. This network configuration is %%%     loosely analogous to general purpose networks where a number of computers %%%     are linked together typically for data sharing but also command and control. %%%     Because of this vehicle cyber security has grown from and is considered to be a %%%     branch of the wider cyber security industry. As such many of the tools are %%%     derived from those used in general purpose computer networks. Vehicle cyber %%%     security tools include: data traffic pattern analysis, honey pots, fingerprinting, %%%     traffic rate monitoring, traffic contextualization, access firewalling, %%%     man-in-the-middle attacks, message destructors.
%%%     
%%%     Vehicle networks tend to differ from general purpose computer networks in the %%%     use unauthenticated message traffic driven by the need for real time critical %%%     command and control messaging. Most general purpose networks will require %%%     authentication before allowing message traffic to flow into nodes. This %%%     authentication is a natural point to implement cyber security. In addition, while the %%%     applications that run on general purpose networks can be very comprehensive, %%%     the code base runs on a limited variety of operating systems that can be %%%     monitored for irregularities by a broad and sophisticated industrial base of cyber %%%     security expertise. Many vehicle networks use single message commands that come %%%     from highly proprietary embed applications with a wide variety of known and %%%     unknown vulnerabilities and with only ad hoc attention to cyber security. %%%     Because there is no enforced authentication, any compromised system on a vehicle %%%     network can be widely used to propagate threats with real time consequences.  %%%     When used together and implemented in a way that reflects the more application %%%     specific aspects of the vehicle cyber threat space, the tools listed can be %%%     effective. When used in a manner that is relevant for general purpose computer %%%     networks but not the vehicle networks these tools can end up only providing a token %%%     level of protection.  There are a number of companies providing vehicle cyber %%%     security solutions (NVIDIA, Harman, IBM, Dellfer, DENSO, etc.). Each company %%%     uses a selection of cyber security tools including some of the techniques listed. %%%     The problem is there is currently no method to evaluate how resilient each %%%     solution is to even the minimalist known threat space.  %%%     \subsection{Implementing cyber threats on desktop systems like Toyota PASTA}
%%%     Toyota PASTA (Portable Automotive Security Testbed with Adaptability) is a %%%     desktop system that emulates a functioning vehicle data network using various %%%     preprogrammed modules and a range of operator inputs to these modules. %%%     PASTA is meant to emulate vehicle networks found on civilian light vehicles, %%%     such as cars. The modules take the operator inputs and use these to generate %%%     vehicle network messages that reflect what would typically be seen on an %%%     operating vehicle. As such it has a library of defined messages many of which are %%%     similar to what is seen on MGVs. Because of this many of the cyber threats that %%%     can be implemented on MGVs can also be implemented on PASTA.  
%%%     

==> includes/introduction_a.tex <==
\section{Prior Work}
% \section{Introduction}
The vulnerabilities of modern vehicles to cyber-attacks through the
\ac{CAN} bus has been demonstrated and studies by several
researchers.\cite{
	hoppe2007sniffing,
	pan2017cyber,
	quintino2017protection,
	bozdal2018hardware,
	bozdal2020evaluation}
Along with the realization that perfect security is impractical, there have
been many calls for systems to be resilient against
cyber-attack.\cite{
	obama2011ppd-8,
	obama2013ppd-21,
	alexeev2017constructing}
Many have offered frameworks and solutions to improve cyber
resilience.\cite{
	bodeau2011framework,
	bodeau2013controls,
	graubart2016observations,
	bodeau2018catalog,
	bodeau2018metrics,
	bodeau2018practice,
	bozdal2020evaluation}
In order for the field of cyber resilience to mature,
there must be ``techniques, tools, and processes for objectively
measuring the attributes of phenomena occurring in the systems of
that discipline.''\cite{kott2021improve}
This paper describes an effort to construct an experimental environment
that will provide data that may be used to develop a quantitative
measurement of cyber resilience.

\subsection{Research Questions}
This report begins the process of answering the following research
question:  ``Is it possible to construct an inexpensive experimental
environment that will produce data of high enough quality to demonstrate a
quantitative measurement for cyber-resilience?''
This measurement must be independent, rigorous, science-based,
repeatable, automated and affordable.
Kott and Linkov spelled out four characteristics of such a measurement.
(a) It must be repeatable---if the same system is measured with the
same tool, the results should be similar.
(b) It must be consistent with respect to missions---similar
missions should yield similar results.
(c) It should have monotonicity with respect to defenses---if 
the defenses are strengthened, then the score should improve.
(d) It should have monotonicity with respect to attacks---if
the threat increases, then the score should
decrease\cite{kott2021improve}.

\subsection{Contribution}


\subsection{Organization}
The development of a quantitative measure of cyber resilience begins
with a clear definition of cyber resilience.
In Section~\ref{sec:background}, we review several of the definitions
of resilience.
In addition, the measure development will require a measurement
methodology.
Section~\ref{sec:background} will also review several of the currently
proposed measurement methodologies for cyber resilience.
Our approach and assumptions are presented in Section~\ref{sec:approach}.
Our results and lessons learned are presented in
Section~\ref{sec:results}.
In Section~\ref{sec:conclusion}, we provide our conclusions and outline
the next steps for developing a quantitative measure of cyber resilience.




==> includes/introduction_b.tex <==
\section{Introduction}
The vulnerabilities of modern vehicles to cyber-attacks through the
\ac{CAN} bus has been demonstrated and studies by several
researchers.\cite{
	hoppe2007sniffing,
	pan2017cyber,
	quintino2017protection,
	bozdal2018hardware,
	bozdal2020evaluation}
Along with the realization that perfect security is impractical, there have
been many calls for systems to be resilient against
cyber-attack.\cite{
	obama2011ppd-8,
	obama2013ppd-21,
	alexeev2017constructing}
Many have offered frameworks and solutions to improve cyber
resilience.\cite{
	bodeau2011framework,
	bodeau2013controls,
	graubart2016observations,
	bodeau2018catalog,
	bodeau2018metrics,
	bodeau2018practice,
	bozdal2020evaluation}
In order for the field of cyber resilience to mature,
there must be "techniques, tools, and processes for objectively
measuring the attributes of phenomena occurring in the systems of
that discipline.''\cite{kott2021improve}
This paper describes an effort to construct an experimental environment
that will provide data that may be used to develop a quantitative
measurement of cyber resilience.

\subsection{Research Questions}
This report begins the process of answering the following research
question:  ``Is it possible to construct an inexpensive experimental
environment that will produce data of high enough quality to demonstrate a
quantitative measurement for cyber-resilience?''
This measurement must be independent, rigorous, science-based,
repeatable, automated and affordable.
Kott and Linkov spelled out four characteristics of such a measurement.
(a) It must be repeatable---if the same system is measured with the
same tool, the results should be similar.
(b) It must be consistent with respect to missions---similar
missions should yield similar results.
(c) It should have monotonicity with respect to defenses---if 
the defenses are strengthened, then the score should improve.
(d) It should have monotonicity with respect to attacks---if
the threat increases, then the score should
decrease\cite{kott2021improve}.

\subsection{Contribution}
This paper describes an inexpensive experimental environment that may be 
used to test various malware and bonware on the \ac{CAN} bus of a modern
vehicle.
A case study is presented and the data from that case study is used to 
measure the cyber resilience of the simulated vehicle. 

\subsection{Organization}
The development of a quantitative measure of cyber resilience begins
with a clear definition of cyber resilience.
In Section~\ref{sec:background}, we review several of the definitions
of resilience.
Our approach and assumptions are presented in Section~\ref{sec:approach}.
Our results and lessons learned are presented in
Section~\ref{sec:results}.
In Section~\ref{sec:conclusion}, we provide our conclusions and outline
the next steps for developing a quantitative measure of cyber resilience.


==> includes/maf.tex <==
\subsection{Mathematical Modeling} \label{sec:maf}
%%%     \begin{figure}
%%%       \aaa{attacks_and_defenses.pdf}
%%%       \caption{System functionality.}
%%%     \end{figure}
In \cite{mmcr} we develop a model for the behavior of a
system's functionality over the course of an incident where it is
being attacked by malware and defended by bonware.  First, we assume
that there is an observable, sufficiently smooth function representing mission
accomplishment, and we define functionality to be its time
derivative.  Thus,
\begin{equation}
  \label{eq:ma}
  F(t) = \frac{d \ma }{dt}, \quad \ma(t) = \int_{t_0}^t F(\tau) \, d\tau.
\end{equation}
The normal
functionality, when the system performs normally and does not
suffer a cyber attack, may, in general, vary with time.
For simplicity, throughout the paper, we assume the normal
functionality to be constant in time, $F_0(t)=\Fnominal.$ 


==> includes/mission_accomplishment_functionality.tex <==
\section{Mathematical Modeling}
%%%     \begin{figure}
%%%       \aaa{attacks_and_defenses.pdf}
%%%       \caption{System functionality.}
%%%     \end{figure}
In \cite{mmcr} we develop a model for the behaviour of a
system's functionality over the course of an incident where it is
being attacked by malware and defended by bonware.  First, we assume
that there is an observable, sufficiently smooth function representing mission
accomplishment, and we define functionality to be its time
derivative.  Then, we briefly discuss the use of area under the curve
(AUC) as a measure of cyber resilience.  
\subsection{Mission Accomplishment and Functionality}
\label{sec:maf}
We define functionality, $F(t),$ to be the time
derivative of mission accomplishment \cite{mmcr}.  Thus
\begin{equation}
  \label{eq:ma}
  F(t) = \frac{d \ma }{dt}, \quad \ma(t) = \int_{t_0}^t F(\tau) \, d\tau.
\end{equation}
The normal
functionality, when the system performs normally and does not
suffer a cyber attack, may, in general, vary with time.
For simplicity, throughout the paper, we assume the normal
functionality to be constant in time, $F_0(t)=\Fnominal.$ 

==> includes/oanalysis.tex <==
\section{Case Study Analysis}


Figure~\ref{fig:fuel-efficiency} (left panels) shows the observed fuel efficiency plotted over the mission duration. The light blue line represents the observed fuel efficiency under the baseline scenario during which no attacks took place. The dotted red line represents the fuel efficiency under two separate attack scenarios, with attacks occurring at $283~s$ and $619~s,$ respectively. The effects of the attacks can be seen starting around $307~s$ and $669~s,$ when the blue and red lines diverge. The loss of fuel efficiency, shaded orange, is the net effect of the attack on fuel efficiency. 

One peculiarity of the fuel efficiency metric is that efficiency in the attack scenario sometimes exceeds that under the baseline scenario after the attack has concluded (around $500~s$ in the top left panel). This behavior is a result of the fact that the engine coolant temperature takes an extended amount of time to return to normal operating temperatures from the $60^\circ\text{C}$ steady state observed while the fan controller is attacked. During this time period in the attack scenario, the fan is not needed. In contrast, the baseline scenario still regularly turns the fan on, during which its average fuel efficiency is adversely affected. Thus, a temporary period of increased average fuel efficiency is observed in the attack scenario. 

In order to quantify the effect of the malware attack, we must consider whether the performance metric is compensatory or non-compensatory. With a compensatory metric, high performance at one time may compensate for lower performance at another time. This may be the case for fuel efficiency if our primary criterion is whether the vehicle completes its mission, or how much fuel is used in total. In that case, the outcome may be computed as the area under the curve (AUC) of performance over time. For attack scenario~1 (attack at $t = 283$), the loss in AUC was 1\% and in attack scenario~2 (attack at $t = 619$) it was 2\% (note that this attack occurred near the end of the mission so there was no time to compensate).

With a non-compensatory metric, high performance at one time does not make up for reduced performance at another time. In the current example, this may be the case if a period of reduced fuel efficiency causes an operator to call in a need to refuel or to signal an expected delay to their destination, causing further negative externalities. In such a case, we should ignore periods of higher-than-nominal performance and instead compute the AUC for an attack scenario as the area under the curve described by the minimum of the baseline and attack scenarios at each time point. Using this calculation, the resulting loss in AUC due to the attack was 2\% in both attack scenarios.

In a second step, the experimental data were analyzed using the novel mathematical framework detailed in a companion paper \cite{mmcr}. Briefly, the framework is used to express the functionality of a vehicle over mission time in terms of a parameterized change process. The key parameters are the impact $M$ of malware and the impact $B$ of so-called bonware (the totality of physical and cyber features that allow a system to resist and recover from cyber compromise). Since the effect of malware is not immediate, the effective onset of malware is modeled as an additional free parameter $t^m$.

The process model is governed by the differential equation $\frac{dF}{dt} = \left(\Fnominal-F(t)) \right) \bonware(t) - F(t) \malware(t) A(t) u(t-t^m)$, where $u(\cdot)$ is the unit step function, which takes the value $0$ if its argument is negative and $1$ otherwise. $F_N$ indicates normative functionality and is set to $1$ in this example. $A(t)$ is $1$ if malware is active at time $t$ and $0$ otherwise.

The process is applied to the functionality $F(t)$ of the vehicle over mission time. Functionality at time $t$ is defined as the ratio of a vehicular performance metric (here, fuel efficiency) at time $t$ in the attack scenario divided by the same metric at time $t$ in either the baseline scenario or the attack scenario, whichever is lower (i.e., $F(t)$ is non-compensatory). Note that due to the high variability of fuel efficiency over short time intervals, the time series was first smoothed with a $72~s$ moving average window before taking the ratio (Fig.~\ref{fig:fuel-efficiency}, left panels).

The parameters of the model can be estimated from data using standard model fitting tools. Our implementation relied on the Monte Carlo estimation of a hidden Markov model as described in \cite{mmcr}. For the current data, we estimated $M = 0.008$, $B = 0.048$, and $t^m = 307~s$ for the first scenario and $M = 0.008$, $B = 0.046$, and $t^m = 669~s$ for the second. These model-based results allow us to quantify the relative impact of malware and bonware among different mission scenarios, vehicles, or attack and defense modalities.

Figure~\ref{fig:fuel-efficiency} (right panels) shows the functionality over time (solid light blue line) for the two case studies. Also shown is the functionality predicted by the three-parameter differential equation model (dashed black line). The model captures the salient aspects of the data well.

\begin{figure*}
  \aaa{fuel_efficiency_11.pdf}
  \aaa{fuel_efficiency_21.pdf}\\
  \aaa{fuel_efficiency_12.pdf}
  \aaa{fuel_efficiency_22.pdf}
  \caption{Describe these fuel efficiency figures.}
  \label{fig:fuel-efficiency}
\end{figure*}


==> includes/oprior_work.tex <==
\section{Prior Work}

There has been a vast amount written about cyber resilience.  Some of
it is qualitative, for example \cite{alexeev}, \cite{henshel}.
Lately, there
has been a growing interest in the quantitative measurement of cyber resilience
\cite{kott2019cyber,kott2017assessing,ligo2021how,linkov2013resilience,mmcr}. 

% \section{Introduction}
The vulnerabilities of modern vehicles to cyber-attacks through the
\ac{CAN} bus has been demonstrated and studies by several
researchers.\cite{
	hoppe2007sniffing,
	pan2017cyber,
	quintino2017protection,
	bozdal2018hardware,
	bozdal2020evaluation}
Along with the realization that perfect security is impractical, there have
been many calls for systems to be resilient against
cyber-attack.\cite{
	obama2011ppd-8,
	obama2013ppd-21,
	alexeev2017constructing}
Many have offered frameworks and solutions to improve cyber
resilience.\cite{
	bodeau2011framework,
	bodeau2013controls,
	graubart2016observations,
	bodeau2018catalog,
	bodeau2018metrics,
	bodeau2018practice,
	bozdal2020evaluation}
In order for the field of cyber resilience to mature,
there must be ``techniques, tools, and processes for objectively
measuring the attributes of phenomena occurring in the systems of
that discipline.''\cite{kott2021improve}
This paper describes an effort to construct an experimental environment
that will provide data that may be used to develop a quantitative
measurement of cyber resilience.

\subsection{Research Questions}
This report begins the process of answering the following research
question:  ``Is it possible to construct an inexpensive experimental
environment that will produce data of high enough quality to demonstrate a
quantitative measurement for cyber-resilience?''
This measurement must be independent, rigorous, science-based,
repeatable, automated and affordable.
Kott and Linkov spelled out four characteristics of such a measurement.
(a) It must be repeatable---if the same system is measured with the
same tool, the results should be similar.
(b) It must be consistent with respect to missions---similar
missions should yield similar results.
(c) It should have monotonicity with respect to defenses---if 
the defenses are strengthened, then the score should improve.
(d) It should have monotonicity with respect to attacks---if
the threat increases, then the score should
decrease\cite{kott2021improve}.

\subsection{Contribution}
\color{blue} What is our contribution?\color{black}


==> includes/portable_testbed.tex <==
\subsection{Portable Automotive Security Testbed with Adaptability}
PASTA, created by Toyota, is a vehicle security testbed designed to
allow researchers the ability to develop and evaluate new security
technology and approaches on realistic “white-box” ECUs [1]. There are
three vehicle ECUs within the testbed, each encompassing a family of
functionality and sitting on their own CAN bus: powertrain, body, and
chassis. These three ECUs are responsible for their respective group
of messages, each generating and responding to traffic on their bus. A
fourth ECU, the central gateway (CGW), acts as a junction between the
three previously mentioned buses. Based on the message and source bus,
the CGW ferries messages to their appropriate destination bus. The
firmware for all ECUs is open-source, and is accompanied by an IDE
from Toyota to promote ease of customization.  PASTA has simulation
boards integrated into the testbed which calculate how the current CAN
messages on the buses would influence a commercial vehicle. These
boards then update the vehicle ECUs with appropriate values. For
example, when acceleration pedal operation is inputted, the chassis
ECU sends a message with the indicated value as a percent. The
simulation boards observe this message and calculate the physics that
would result from the input. The results are used to update the values
reported by the powertrain ECU, which it outputs onto its bus. In this
instance, the powertrain ECU would send messages indicating the new
engine throttle position, RPM, and vehicle speed. The simulation
boards are connected directly to the vehicle ECUs via a serial port on
each ECU board, so the physics data is not mixed with messages on the
CAN bus.  An issue with the simulation boards is that they are
essentially “black-boxes” and closed-source. We cannot alter, for
instance, the parameters involving the engine (e.g., torque and
horsepower), the weight of the vehicle, or the terrain that the boards
are assuming is being traversed. To counteract this issue, we
integrated a simulation engine that would allow for user-defined
vehicle details as well as a custom terrain. In this configuration,
PASTA becomes hardware-in-the-loop for the simulation engine. Attacks
or defenses that affect the ECUs present in PASTA will also affect the
vehicle within simulation. This is essential in order to observe
realistic threats and defenses and their effects on vehicle
performance.


==> includes/unity_3d.tex <==
\subsection{Unity 3D}
\subsubsection{Simulated Light Military Vehicle}

We implemented a light military vehicle within Unity3D designed to
interface with data inputs from the white-box ECUs within PASTA. In
general, the vehicle produces inputs in response to the simulated
terrain. These inputs are sent to the corresponding ECUs within PASTA
as if they were generated by PASTA itself. We then send responses to
these inputs from the ECUs back to the simulated vehicle, which it
uses to calculate things like torque and fuel consumption. For
example, assume that the vehicle reports that the accelerator is set
to 50\%. This message is injected into PASTA as if the chassis ECU had
generated it. The powertrain ECU responds to the message with the
corresponding amount of engine throttle. A message with the engine
throttle is sent back to the vehicle, which is then applied to engine
power calculations. With this data flow, any attacks present on the
ECUs within PASTA will affect the simulated vehicle.  An automated
driver is responsible for generating steering, acceleration, and
braking inputs as the vehicle traverses the simulated
terrain. Steering is guided by the use of a waypoint system. Both
acceleration and braking inputs are calculated via a
proportional-integral-derivative (PID) controller. The controller
prevents oscillation in the acceleration and braking inputs, and
reliably responds to sudden changes in the terrain.  Engine
performance is calculated through the use of torque, horsepower, and
brake-specific fuel consumption (BSFC) curves. Engine RPM is derived
using the vehicle speed, wheel circumference, and effective gear
ratio. Using this RPM value, the curves are evaluated to discern the
corresponding torque, horsepower, and a BSFC value. Torque is
multiplied by the throttle and the current effective gear ratio to
obtain the total amount of torque that can be applied to the
wheels. Since our vehicle is All-Wheel Drive (AWD), each wheel
receives the total amount of torque divided by the number of wheels on
the vehicle, which is six in this case. Horsepower and the BSFC value
are used in conjunction to calculate the amount of fuel that has been
used each time the physics engine undergoes an update. Based upon the
torque curve, optimal gear shift points were calculated. The resulting
shift points, being optimal in terms of torque output, confer an
aggressive acceleration profile for the vehicle.  The vehicle is
capable of providing sensor information that is either not present in
PASTA or needs its functionality altered for our purposes. Currently,
this applies to the engine coolant temperature. Engine temperature is
present in PASTA, but is aligned to the temperature characteristics of
a commercial sedan. Within Unity3D, we implemented a basic temperature
model that can be controlled by an external fan controller ECU. The
fan controller, described in a later section, monitors the temperature
reported by the vehicle. Once it hits an upper threshold, it activates
the simulated fan, which begins to lower the temperature. The fan
itself takes around 50 horsepower to operate, which results in an
approximate 25\% drop in the available torque that can be applied to
the wheels.
\subsubsection{Terrain}
\begin{itemize}
\item About 151 km
\item Variety of course types
\item Main road, off road, incline,
  decline, hilly
\item Contains trigger points that set the target speed of
  the vehicle depending on the course type
\item Off road $\to$40 kph
\item Main road $\to$60 kph
\end{itemize}
\subsubsection{Reportable Data}
\begin{itemize}
\item Reproduce and clean up table from BoD slides
\item May have to span two columns at the top of a page
\item Mention the parameters that are configurable to produce
  statistically significant data
  \begin{itemize}
  \item 5 different subroutes
  \item Variable/random attack times
  \item In the future, two additional vehicle types
  \end{itemize}
\end{itemize}
